Edge Dithering for Robust Adaptive Graph Convolutional Networks

Graph convolutional networks (GCNs) are vulnerable to perturbations of the graph structure that are either random, or, adversarially designed. The perturbed links modify the graph neighborhoods, which critically affects the performance of GCNs in semi-supervised learning (SSL) tasks. Aiming at robustifying GCNs conditioned on the perturbed graph, the present paper generates multiple auxiliary graphs, each having its binary 0-1 edge weights flip values with probabilities designed to enhance robustness. The resultant edge-dithered auxiliary graphs are leveraged by an adaptive (A)GCN that performs SSL. Robustness is enabled through learnable graph-combining weights along with suitable regularizers. Relative to GCN, the novel AGCN achieves markedly improved performance in tests with noisy inputs, graph perturbations, and state-of-the-art adversarial attacks. Further experiments with protein interaction networks showcase the competitive performance of AGCN for SSL over multiple graphs.

==> figs/misc/gcntikz.tex <==
\begin{tikzpicture}[scale=0.7, transform shape]
\definecolor{paramcolor}{HTML}{50ae55}
\definecolor{inputcolor}{HTML}{fd9727}
\definecolor{outputcolor}{HTML}{f1453d}
\tikzset{
	inputmat/.style = {rectangle, draw=inputcolor!70, fill=inputcolor!40, thick, minimum width=1.4cm, minimum height = 1cm},
	outputmat/.style = {rectangle, draw=outputcolor!0, fill=outputcolor!50, thick, minimum width=0.6cm, minimum height = 1.0cm},
	thickermat/.style = {rectangle, draw=black!50, fill=black!20, thick, minimum width=1.4cm, minimum height = 1cm},
	parameter/.style = {rectangle, draw=paramcolor!70, fill=paramcolor!40, thick, minimum width=0.6cm, minimum height = 1.4cm},
}
\node [inputmat](x) [draw] { }; 
\node [above =0cm of x] (xlabel) {$H^{(i-1)}$ }; 
%\node [below of=x](xlabel) {$H^{(l)}$}
\node [draw, below of=x](mult) {$\times$};
\node [left of=mult] (a) {$\widehat{A}$};
%\node [thickermat, below of=mult](ax) [draw] {}; 
\node [draw, below of=mult](wmult) {$\times$};
\node [parameter, right =0.55cm of wmult](w) {};
\node [below=0cm of w](wl) {$W^{(i)}$}; % 
\node [outputmat, below of=wmult](y) {};
\node [below =0cm of y] (xlabel) {$H^{(i)}$ }; 
%\node [draw, right of=wmult](sigma) {$\sigma$};


\draw[-{>}] (x) -- (mult);
\draw[-{>}] (a) -- (mult);
%\draw[-{>}] (mult) -- (ax);
\draw[-{>}] (mult) -- (wmult);
\draw[-{>}] (w) -- (wmult);
\draw[-{>}] (wmult) -- (y);
\end{tikzpicture}


==> figs/misc/kipf.tex <==
%% Creator: Inkscape inkscape 0.92.2pre0, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'kipf.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{472.39506759bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,.9)%
    \put(0,0.1){\includegraphics[width=\unitlength,page=1]{figs/kipf1.pdf}}%
    
    {\fontsize{100pt}{120pt} \put(0.53,0.4){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$W^{(i)}$ }}}}%

    {\fontsize{100pt}{120pt} \put(0.7,0.8){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\hat{A} H^{(i)}$ }}}}%
    
    {\fontsize{100pt}{120pt} \put(0.48,0.15){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$H^{(i+1)}$ }}}}%

    {\fontsize{100pt}{120pt} \put(0.26,0.0){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$H^{(i+1)} = \sigma(\hat{A} H^{(i)} W^{(i)})$ }}}}%
  \end{picture}%
\endgroup%


==> figs/misc/learned_cora.tex <==
\begin{tikzpicture}[scale=0.6, transform shape]
\definecolor{paramcolor}{HTML}{50ae55}
\definecolor{inputcolor}{HTML}{fd9727}
\definecolor{outputcolor}{HTML}{f1453d}


% Height scale = 7 = 0.1

\tikzset{
	inputmat/.style = {rectangle, draw=inputcolor!70, fill=inputcolor!40, thick, minimum width=1.4cm, minimum height = 1cm},
	output1mat2/.style = {rectangle, draw=outputcolor!90, fill=outputcolor!70,  line width=0.1mm, inner sep=0pt, minimum width=1.0cm, minimum height = 0cm},
	output2mat2/.style = {rectangle, draw=outputcolor!90, fill=outputcolor!30, line width=0.1mm, inner sep=0pt, minimum width=1.0cm, minimum height = 0.1cm},
	output3mat2/.style = {rectangle, draw=outputcolor!90, fill=outputcolor!50, line width=0.1mm, inner sep=0pt, minimum width=1cm, minimum height = 0.1cm},
	output1mat1/.style = {rectangle, draw=outputcolor!90, fill=outputcolor!70, line width=0.1mm, inner sep=0pt, minimum width=1.4cm, minimum height = 0.343cm},
	output2mat1/.style = {rectangle, draw=outputcolor!90, fill=outputcolor!30, line width=0.1mm, inner sep=0pt, minimum width=1.4cm, minimum height = 0.257cm},
	output3mat1/.style = {rectangle, draw=outputcolor!90, fill=outputcolor!50, line width=0.1mm, inner sep=0pt, minimum width=1.4cm, minimum height = 0.257cm},
	thickermat/.style = {rectangle, draw=black!50, fill=black!20, thick, minimum width=1.4cm, minimum height = 1cm},
	thinmat/.style = {rectangle, draw=black!50, fill=black!20, thick, minimum width=0.2cm,
		minimum height = 1cm},
	parameter_1_1/.style = {rectangle, draw=paramcolor!70, fill=paramcolor!40, thin, minimum width=1cm, minimum height = 0.343cm}, % 24
	parameter_1_2/.style = {rectangle, draw=paramcolor!70, fill=paramcolor!40, thin, minimum width=1cm, minimum height = 0.257cm}, % 18
	parameter_1_3/.style = {rectangle, draw=paramcolor!70, fill=paramcolor!40, thin, minimum width=1cm, minimum height = 0.257cm}, % 18
	parameter_2_1/.style = {rectangle, inner sep=0pt, draw=paramcolor!70, fill=paramcolor!40, thin, minimum width=0.7cm, minimum height = 0.0cm},   % 0
	parameter_2_2/.style = {rectangle, inner sep=0pt, draw=paramcolor!70, fill=paramcolor!40, thin, minimum width=0.7cm, minimum height = 0.1cm},   % 35
	parameter_2_3/.style = {rectangle, draw=paramcolor!70, fill=paramcolor!40, thin, minimum width=0.7cm, minimum height = 0.1cm},   % 21
}
\node [inputmat,anchor=east](x) [draw] {}; 
\node [below=-0.5cm, left=0.45cm] (a) {$X$};
\draw [line width=0.1mm] ($(x.north west) + (-0.1,0) $ ) -- ($(x.south west) - (0.1,0.0)$); % vertical line
\draw [line width=0.1mm] ($(x.north west) + (-0.13,0) $ ) -- ($(x.north west) + (-0.07,0)$); % top tick
\draw [line width=0.1mm] ($(x.south west) + (-0.13,0) $ ) -- ($(x.south west) + (-0.07,0)$); % bottom tick
\node [left=0.0cm of x]()[]{\tiny $^{1433}$}; % left label

\draw [line width=0.1mm] ($(x.north west) + (0,0.1) $ ) -- ($(x.north east) + (0,0.1)$); % horizontal line
\draw [line width=0.1mm] ($(x.north west) + (0,0.07) $ ) -- ($(x.north west) + (0,0.13)$); % left tick
\draw [line width=0.1mm] ($(x.north east) + (0,0.07) $ ) -- ($(x.north east) + (0,0.13)$); % bottom tick
\node [above=-0.05cm of x]()[]{\tiny $^{n=2708}$}; % top label

%\node [right=-0.4em of x] (xlabel) {$H^{(l-1)}$};
%\node [below of=x](xlabel) {$H^{(l)}$}

\draw [decorate,decoration={brace,amplitude=2.5pt,mirror,raise=1ex}]
   ($ (x.south east)+(-0.8em, -0.5em) $) -- ($(x.north east)+(-0.8em, 0.5em)$) node[midway,yshift=0em]{};



%%%%%%%%%%%%%%%%%%%% LAYER 1

% Nodes
% POW 0
\node [draw, above right=0.7cm and 0.5cm of x](mult) {$\times$};
\node [below=0cm of mult] (a) {$\widehat{A}^0$};
\node [draw, right= 1cm of mult](wmult) {$\times$};
\node [parameter_1_1, above=0.25cm of wmult](w) {};
\draw [line width=0.1mm] ($(w.north west) + (0,0.1) $ ) -- ($(w.north east) + (0,0.1)$); % horizontal line
\draw [line width=0.1mm] ($(w.north west) + (0,0.07) $ ) -- ($(w.north west) + (0,0.13)$); % left tick
\draw [line width=0.1mm] ($(w.north east) + (0,0.07) $ ) -- ($(w.north east) + (0,0.13)$); % bottom tick
\node [above=-0.05cm of w]()[]{\tiny $^{1433}$}; % top label

\draw [line width=0.1mm] ($(w.north east) + (0.1,0) $ ) -- ($(w.south east) + (0.1,0.0)$); % vertical line
\draw [line width=0.1mm] ($(w.north east) + (0.13,0) $ ) -- ($(w.north east) + (+0.07,0)$); % top tick
\draw [line width=0.1mm] ($(w.south east) + (0.13,0) $ ) -- ($(w.south east) + (+0.07,0)$); % bottom tick
\node [right=0.0cm of w]()[]{\tiny $^{24}$}; % right label
\node[left=-0.15cm of w] {\tiny $^{W^{(1)}_0}$};


% Edges
\draw ($(x.east) + (0.2em, 0em)$) edge[out=0,in=180,->] (mult);
%\draw[-{>}] (a) -- (mult);
\draw[-{>}] (mult) -- (wmult);
\draw[-{>}] (w) -- (wmult);


% POW 1
\node [draw, right=0.5cm of x](mult1) {$\times$};
\node [below=0cm of mult1] (a1) {$\widehat{A}^1$};
\node [draw, right=1cm of mult1](wmult1) {$\times$};
\node [parameter_1_2, above=0.25cm of wmult1](w1) {};
\node [output2mat1, right=1.3cm of wmult1](yy1) {};


\draw [line width=0.1mm] ($(w1.north east) + (0.1,0) $ ) -- ($(w1.south east) + (0.1,0.0)$); % vertical line
\draw [line width=0.1mm] ($(w1.north east) + (0.13,0) $ ) -- ($(w1.north east) + (+0.07,0)$); % top tick
\draw [line width=0.1mm] ($(w1.south east) + (0.13,0) $ ) -- ($(w1.south east) + (+0.07,0)$); % bottom tick
\node [right=0.0cm of w1]()[]{\tiny $^{18}$}; % right label
\node[left=-0.15cm of w1] {\tiny $^{W^{(1)}_1}$};

% Edges
\draw ($(x.east) + (0.2em, 0em)$) edge[out=0,in=180,->] (mult1);
%\draw[-{>}] (a1) -- (mult1);
\draw[-{>}] (mult1) -- (wmult1);
\draw[-{>}] (w1) -- (wmult1);
\draw (wmult1) edge[out=0,in=180,->] (yy1);


% POW 2
\node [draw, below right=0.7 and 0.5cm of x](mult2) {$\times$};
\node [below=0cm of mult2] (a2) {$\widehat{A}^2$};
\node [draw, right=1cm of mult2](wmult2) {$\times$};
\node [parameter_1_3, above=0.25cm of wmult2](w2) {};

\draw [line width=0.1mm] ($(w2.north east) + (0.1,0) $ ) -- ($(w2.south east) + (0.1,0.0)$); % vertical line
\draw [line width=0.1mm] ($(w2.north east) + (0.13,0) $ ) -- ($(w2.north east) + (+0.07,0)$); % top tick
\draw [line width=0.1mm] ($(w2.south east) + (0.13,0) $ ) -- ($(w2.south east) + (+0.07,0)$); % bottom tick
\node [right=0.0cm of w2]()[]{\tiny $^{18}$}; % right label
\node[left=-0.15cm of w2] {\tiny $^{W^{(1)}_2}$};


% Edges
\draw ($(x.east) + (0.2em, 0em)$) edge[out=0,in=180,->] (mult2);
\draw[-{>}] (mult2) -- (wmult2);
\draw[-{>}] (w2) -- (wmult2);



%% OUTPUTS

\node [output1mat1, above=0.1em of yy1](yy) {};
\draw (wmult) edge[out=0,in=180,->] (yy);
\node [output3mat1, below=0.1em of yy1](yy2) {};
\draw (wmult2) edge[out=0,in=180,->] (yy2);

\draw [line width=0.1mm] ($(yy.north west) + (0,0.1) $ ) -- ($(yy.north east) + (0,0.1)$); % horizontal line
\draw [line width=0.1mm] ($(yy.north west) + (0,0.07) $ ) -- ($(yy.north west) + (0,0.13)$); % left tick
\draw [line width=0.1mm] ($(yy.north east) + (0,0.07) $ ) -- ($(yy.north east) + (0,0.13)$); % bottom tick
\node [above=-0.05cm of yy]()[]{\tiny $^n$}; % top label

\draw [line width=0.1mm] ($(yy.north east) + (-0.1,0) $ ) -- ($(yy2.south east) - (0.1,0.0)$); % vertical line
\draw [line width=0.1mm] ($(yy.north east) + (-0.13,0) $ ) -- ($(yy.north east) + (-0.07,0)$); % top tick
\draw [line width=0.1mm] ($(yy2.south east) + (-0.13,0) $ ) -- ($(yy2.south east) + (-0.07,0)$); % bottom tick
\node [right=-0.5cm of yy1]()[]{\tiny $^{60}$}; % left label



%%%%%%%%%%%%%%%%%%%% LAYER 2



\draw [decorate,decoration={brace,amplitude=2.5pt,mirror,raise=1ex}]
($ (yy2.south east)+(-0.8em, -0.65em) $) -- ($(yy.north east)+(-0.8em, 0.45em)$) node[midway,yshift=0em]{};


% Pow 0
\node [draw, above right=1.2cm and 0.5cm of yy1](qmult) {$\times$};
\node [below=0cm of qmult] (qa) {$\widehat{A}^0$};
\node [draw, right=1cm of qmult](qwmult) {$\times$};
\node [parameter_2_1, above=0.25cm of qwmult](qw) {};
\draw [line width=0.1mm] ($(qw.north west) + (0,0.1) $ ) -- ($(qw.north east) + (0,0.1)$); % horizontal line
\draw [line width=0.1mm] ($(qw.north west) + (0,0.07) $ ) -- ($(qw.north west) + (0,0.13)$); % left tick
\draw [line width=0.1mm] ($(qw.north east) + (0,0.07) $ ) -- ($(qw.north east) + (0,0.13)$); % bottom tick
\node [above=-0.05cm of qw]()[]{\tiny $^{60}$}; % top label
\draw [line width=0.1mm] ($(qw.north east) + (0.1,0.05) $ ) -- ($(qw.south east) + (0.1,-0.05)$); % vertical line
\draw [line width=0.1mm] ($(qw.north east) + (0.13,0.05) $ ) -- ($(qw.north east) + (+0.07,0.05)$); % top tick
\draw [line width=0.1mm] ($(qw.south east) + (0.13,-0.05) $ ) -- ($(qw.south east) + (+0.07,-0.05)$); % bottom tick
\node [right=0.0cm of qw]()[]{\tiny $^{_{0}}$}; % right label
\node[left=-0.15cm of qw] {\tiny $^{W^{(2)}_0}$};



% Edges
\draw ($(yy1.east) + (0.2em, 0em)$) edge[out=0,in=180,->] (qmult);
\draw[-{>}] (qmult) -- (qwmult);
\draw[-{>}] (qw) -- (qwmult);


% POW 1
\node [draw, right=0.5cm of yy1](qmult1) {$\times$};
\node [below=0cm of qmult1] (qa1) {$\widehat{A}^1$};
\node [draw, right=1cm of qmult1](qwmult1) {$\times$};
\node [parameter_2_2, above=0.25cm of qwmult1](qw1) {};
\node [output2mat2, right=1.3cm of qwmult1](qyy1) {};
\draw [line width=0.1mm] ($(qw1.north east) + (0.1,0) $ ) -- ($(qw1.south east) + (0.1,0.0)$); % vertical line
\draw [line width=0.1mm] ($(qw1.north east) + (0.13,0) $ ) -- ($(qw1.north east) + (+0.07,0)$); % top tick
\draw [line width=0.1mm] ($(qw1.south east) + (0.13,0) $ ) -- ($(qw1.south east) + (+0.07,0)$); % bottom tick
\node [right=0.0cm of qw1]()[]{\tiny $^{7}$}; % right label
\node[left=-0.15cm of qw1] {\tiny $^{W^{(2)}_1}$};

% Edges
\draw ($(yy1.east) + (0.2em, 0em)$) edge[out=0,in=180,->] (qmult1);
\draw[-{>}] (qmult1) -- (qwmult1);
\draw[-{>}] (qw1) -- (qwmult1);
\draw (qwmult1) edge[out=0,in=180,->] (qyy1);


% POW 2
\node [draw, below right=1.1 and 0.5cm of yy1](qmult2) {$\times$};
\node [below=0cm of qmult2] (qa2) {$\widehat{A}^2$};
\node [draw, right=1cm of qmult2](qwmult2) {$\times$};
\node [parameter_2_3, above=0.25cm of qwmult2](qw2) {};
\draw [line width=0.1mm] ($(qw2.north east) + (0.1,0) $ ) -- ($(qw2.south east) + (0.1,0.0)$); % vertical line
\draw [line width=0.1mm] ($(qw2.north east) + (0.13,0) $ ) -- ($(qw2.north east) + (+0.07,0)$); % top tick
\draw [line width=0.1mm] ($(qw2.south east) + (0.13,0) $ ) -- ($(qw2.south east) + (+0.07,0)$); % bottom tick
\node [right=0.0cm of qw2]()[]{\tiny $^{7}$}; % right label
\node[left=-0.15cm of qw2] {\tiny $^{W^{(2)}_2}$};


% Edges
\draw ($(yy1.east) + (0.2em, 0em)$) edge[out=0,in=180,->] (qmult2);
\draw[-{>}] (qmult2) -- (qwmult2);
\draw[-{>}] (qw2) -- (qwmult2);



%% OUTPUTS

\node [output1mat2, above=0.1em of qyy1](qyy) {};
\draw (qwmult) edge[out=0,in=180,->] (qyy);
\node [output3mat2, below=0.1em of qyy1](qyy2) {};
\draw (qwmult2) edge[out=0,in=180,->] (qyy2);


\draw [line width=0.1mm] ($(qyy.north west) + (0,0.1) $ ) -- ($(qyy.north east) + (0,0.1)$); % horizontal line
\draw [line width=0.1mm] ($(qyy.north west) + (0,0.07) $ ) -- ($(qyy.north west) + (0,0.13)$); % left tick
\draw [line width=0.1mm] ($(qyy.north east) + (0,0.07) $ ) -- ($(qyy.north east) + (0,0.13)$); % bottom tick
\node [above=-0.05cm of qyy]()[]{\tiny $^n$}; % top label

\draw [line width=0.1mm] ($(qyy.north east) + (0.1,0) $ ) -- ($(qyy2.south east) + (0.1,0.0)$); % vertical line
\draw [line width=0.1mm] ($(qyy.north east) + (0.13,0) $ ) -- ($(qyy.north east) + (0.07,0)$); % top tick
\draw [line width=0.1mm] ($(qyy2.south east) + (0.13,0) $ ) -- ($(qyy2.south east) + (0.07,0)$); % bottom tick
\node [right=0cm of qyy1]()[]{\tiny $^{14}$}; % left label


\end{tikzpicture}


==> figs/misc/learned_pubmed.tex <==

% Layer 1 = 17,23,20
% Layer 2 = 9, 9, 42

\begin{tikzpicture}[scale=0.6, transform shape]
\definecolor{paramcolor}{HTML}{50ae55}
\definecolor{inputcolor}{HTML}{fd9727}
\definecolor{outputcolor}{HTML}{f1453d}


% Height scale = 7 = 0.1

\tikzset{
	inputmat/.style = {rectangle, draw=inputcolor!70, fill=inputcolor!40, thick, minimum width=1.4cm, minimum height = 0.7cm},
	output1mat1/.style = {rectangle, draw=outputcolor!90, fill=outputcolor!70, line width=0.1mm, inner sep=0pt, minimum width=1.4cm, minimum height = 0.243cm},
	output2mat1/.style = {rectangle, draw=outputcolor!90, fill=outputcolor!30, line width=0.1mm, inner sep=0pt, minimum width=1.4cm, minimum height = 0.329cm},
	output3mat1/.style = {rectangle, draw=outputcolor!90, fill=outputcolor!50, line width=0.1mm, inner sep=0pt, minimum width=1.4cm, minimum height = 0.286cm},
	output1mat2/.style = {rectangle, draw=outputcolor!90, fill=outputcolor!70,  line width=0.1mm, inner sep=0pt, minimum width=1.0cm, minimum height = 0.0429cm},
	output2mat2/.style = {rectangle, draw=outputcolor!90, fill=outputcolor!30, line width=0.1mm, inner sep=0pt, minimum width=1.0cm, minimum height = 0.0858cm},
	output3mat2/.style = {rectangle, draw=outputcolor!90, fill=outputcolor!50, line width=0.1mm, inner sep=0pt, minimum width=1cm, minimum height = 0.0429cm},
	thickermat/.style = {rectangle, draw=black!50, fill=black!20, thick, minimum width=1.4cm, minimum height = 1cm},
	thinmat/.style = {rectangle, draw=black!50, fill=black!20, thick, minimum width=0.2cm,
		minimum height = 1cm},
	parameter_1_1/.style = {rectangle, draw=paramcolor!70, fill=paramcolor!40, thin, minimum width=0.7cm, minimum height = 0.243cm}, % 17
	parameter_1_2/.style = {rectangle, draw=paramcolor!70, fill=paramcolor!40, thin, minimum width=0.7cm, minimum height = 0.329cm}, % 23
	parameter_1_3/.style = {rectangle, draw=paramcolor!70, fill=paramcolor!40, thin, minimum width=0.7cm, minimum height =0.286cm}, % 20
	parameter_2_1/.style = {rectangle, inner sep=0pt, draw=paramcolor!70, fill=paramcolor!40, thin, minimum width=0.7cm, minimum height = 0.0429cm},   % 3
	parameter_2_2/.style = {rectangle, inner sep=0pt, draw=paramcolor!70, fill=paramcolor!40, thin, minimum width=0.7cm, minimum height = 0.0858cm},   % 6
	parameter_2_3/.style = {rectangle,
	inner sep=0pt,
	draw=paramcolor!70, fill=paramcolor!40, thin, minimum width=0.7cm, minimum height = 0.0429cm},   % 3   
}
\node [inputmat,anchor=east](x) [draw] {}; 
\node [below=-0.5cm, left=0.45cm] (a) {$X$};
\draw [line width=0.1mm] ($(x.north west) + (-0.1,0) $ ) -- ($(x.south west) - (0.1,0.0)$); % vertical line
\draw [line width=0.1mm] ($(x.north west) + (-0.13,0) $ ) -- ($(x.north west) + (-0.07,0)$); % top tick
\draw [line width=0.1mm] ($(x.south west) + (-0.13,0) $ ) -- ($(x.south west) + (-0.07,0)$); % bottom tick
\node [left=0.0cm of x]()[]{\tiny $^{500}$}; % left label

\draw [line width=0.1mm] ($(x.north west) + (0,0.1) $ ) -- ($(x.north east) + (0,0.1)$); % horizontal line
\draw [line width=0.1mm] ($(x.north west) + (0,0.07) $ ) -- ($(x.north west) + (0,0.13)$); % left tick
\draw [line width=0.1mm] ($(x.north east) + (0,0.07) $ ) -- ($(x.north east) + (0,0.13)$); % bottom tick
\node [above=-0.05cm of x]()[]{\tiny $^{n=19717}$}; % top label

%\node [right=-0.4em of x] (xlabel) {$H^{(l-1)}$};
%\node [below of=x](xlabel) {$H^{(l)}$}

\draw [decorate,decoration={brace,amplitude=2.5pt,mirror,raise=1ex}]
($ (x.south east)+(-0.8em, -0.5em) $) -- ($(x.north east)+(-0.8em, 0.5em)$) node[midway,yshift=0em]{};



%%%%%%%%%%%%%%%%%%%% LAYER 1

% Nodes
% POW 0
\node [draw, above right=0.7cm and 0.5cm of x](mult) {$\times$};
\node [below=0cm of mult] (a) {$\widehat{A}^0$};
\node [draw, right=1cm of mult](wmult) {$\times$};
\node [parameter_1_1, above=0.25cm of wmult](w) {};
\draw [line width=0.1mm] ($(w.north west) + (0,0.1) $ ) -- ($(w.north east) + (0,0.1)$); % horizontal line
\draw [line width=0.1mm] ($(w.north west) + (0,0.07) $ ) -- ($(w.north west) + (0,0.13)$); % left tick
\draw [line width=0.1mm] ($(w.north east) + (0,0.07) $ ) -- ($(w.north east) + (0,0.13)$); % bottom tick
\node [above=-0.05cm of w]()[]{\tiny $^{500}$}; % top label

\draw [line width=0.1mm] ($(w.north east) + (0.1,0) $ ) -- ($(w.south east) + (0.1,0.0)$); % vertical line
\draw [line width=0.1mm] ($(w.north east) + (0.13,0) $ ) -- ($(w.north east) + (+0.07,0)$); % top tick
\draw [line width=0.1mm] ($(w.south east) + (0.13,0) $ ) -- ($(w.south east) + (+0.07,0)$); % bottom tick
\node [right=0.0cm of w]()[]{\tiny $^{17}$}; % right label
\node[left=-0.15cm of w] {\tiny $^{W^{(1)}_0}$};



% Edges
\draw ($(x.east) + (0.2em, 0em)$) edge[out=0,in=180,->] (mult);
%\draw[-{>}] (a) -- (mult);
\draw[-{>}] (mult) -- (wmult);
\draw[-{>}] (w) -- (wmult);


% POW 1
\node [draw, right=0.5cm of x](mult1) {$\times$};
\node [below=0cm of mult1] (a1) {$\widehat{A}^1$};
\node [draw, right=1cm of mult1](wmult1) {$\times$};
\node [parameter_1_2, above=0.25cm of wmult1](w1) {};
\node [output2mat1, right=1.3cm of wmult1](yy1) {};


\draw [line width=0.1mm] ($(w1.north east) + (0.1,0) $ ) -- ($(w1.south east) + (0.1,0.0)$); % vertical line
\draw [line width=0.1mm] ($(w1.north east) + (0.13,0) $ ) -- ($(w1.north east) + (+0.07,0)$); % top tick
\draw [line width=0.1mm] ($(w1.south east) + (0.13,0) $ ) -- ($(w1.south east) + (+0.07,0)$); % bottom tick
\node [right=0.0cm of w1]()[]{\tiny $^{23}$}; % right label
\node[left=-0.15cm of w1] {\tiny $^{W^{(1)}_1}$};


% Edges
\draw ($(x.east) + (0.2em, 0em)$) edge[out=0,in=180,->] (mult1);
%\draw[-{>}] (a1) -- (mult1);
\draw[-{>}] (mult1) -- (wmult1);
\draw[-{>}] (w1) -- (wmult1);
\draw (wmult1) edge[out=0,in=180,->] (yy1);


% POW 2
\node [draw, below right=0.7 and 0.5cm of x](mult2) {$\times$};
\node [below=0cm of mult2] (a2) {$\widehat{A}^2$};
\node [draw, right=1cm of mult2](wmult2) {$\times$};
\node [parameter_1_3, above=0.25cm of wmult2](w2) {};

\draw [line width=0.1mm] ($(w2.north east) + (0.1,0) $ ) -- ($(w2.south east) + (0.1,0.0)$); % vertical line
\draw [line width=0.1mm] ($(w2.north east) + (0.13,0) $ ) -- ($(w2.north east) + (+0.07,0)$); % top tick
\draw [line width=0.1mm] ($(w2.south east) + (0.13,0) $ ) -- ($(w2.south east) + (+0.07,0)$); % bottom tick
\node [right=0.0cm of w2]()[]{\tiny $^{20}$}; % right label
\node[left=-0.15cm of w2] {\tiny $^{W^{(1)}_2}$};


% Edges
\draw ($(x.east) + (0.2em, 0em)$) edge[out=0,in=180,->] (mult2);
\draw[-{>}] (mult2) -- (wmult2);
\draw[-{>}] (w2) -- (wmult2);



%% OUTPUTS

\node [output1mat1, above=0.1em of yy1](yy) {};
\draw (wmult) edge[out=0,in=180,->] (yy);
\node [output3mat1, below=0.1em of yy1](yy2) {};
\draw (wmult2) edge[out=0,in=180,->] (yy2);

\draw [line width=0.1mm] ($(yy.north west) + (0,0.1) $ ) -- ($(yy.north east) + (0,0.1)$); % horizontal line
\draw [line width=0.1mm] ($(yy.north west) + (0,0.07) $ ) -- ($(yy.north west) + (0,0.13)$); % left tick
\draw [line width=0.1mm] ($(yy.north east) + (0,0.07) $ ) -- ($(yy.north east) + (0,0.13)$); % bottom tick
\node [above=-0.05cm of yy]()[]{\tiny $^n$}; % top label

\draw [line width=0.1mm] ($(yy.north east) + (-0.1,0) $ ) -- ($(yy2.south east) - (0.1,0.0)$); % vertical line
\draw [line width=0.1mm] ($(yy.north east) + (-0.13,0) $ ) -- ($(yy.north east) + (-0.07,0)$); % top tick
\draw [line width=0.1mm] ($(yy2.south east) + (-0.13,0) $ ) -- ($(yy2.south east) + (-0.07,0)$); % bottom tick
\node [right=-0.5cm of yy1]()[]{\tiny $^{60}$}; % left label



%%%%%%%%%%%%%%%%%%%% LAYER 2



\draw [decorate,decoration={brace,amplitude=2.5pt,mirror,raise=1ex}]
($ (yy2.south east)+(-0.8em, -0.65em) $) -- ($(yy.north east)+(-0.8em, 0.45em)$) node[midway,yshift=0em]{};


% Pow 0
\node [draw, above right=1.2cm and 0.5cm of yy1](qmult) {$\times$};
\node [below=0cm of qmult] (qa) {$\widehat{A}^0$};
\node [draw, right = 1cm of qmult](qwmult) {$\times$};
\node [parameter_2_1, above=0.25cm of qwmult](qw) {};
\draw [line width=0.1mm] ($(qw.north west) + (0,0.1) $ ) -- ($(qw.north east) + (0,0.1)$); % horizontal line
\draw [line width=0.1mm] ($(qw.north west) + (0,0.07) $ ) -- ($(qw.north west) + (0,0.13)$); % left tick
\draw [line width=0.1mm] ($(qw.north east) + (0,0.07) $ ) -- ($(qw.north east) + (0,0.13)$); % bottom tick
\node [above=-0.05cm of qw]()[]{\tiny $^{60}$}; % top label
\draw [line width=0.1mm] ($(qw.north east) + (0.1,0) $ ) -- ($(qw.south east) + (0.1,0.0)$); % vertical line
\draw [line width=0.1mm] ($(qw.north east) + (0.13,0) $ ) -- ($(qw.north east) + (+0.07,0)$); % top tick
\draw [line width=0.1mm] ($(qw.south east) + (0.13,0) $ ) -- ($(qw.south east) + (+0.07,0)$); % bottom tick
\node [right=0.0cm of qw]()[]{\tiny $^{3}$}; % right label
\node[left=-0.15cm of qw] {\tiny $^{W^{(2)}_0}$};


% Edges
\draw ($(yy1.east) + (0.2em, 0em)$) edge[out=0,in=180,->] (qmult);
\draw[-{>}] (qmult) -- (qwmult);
\draw[-{>}] (qw) -- (qwmult);


% POW 1
\node [draw, right=0.5cm of yy1](qmult1) {$\times$};
\node [below=0cm of qmult1] (qa1) {$\widehat{A}^1$};
\node [draw, right= 1cm of qmult1](qwmult1) {$\times$};
\node [parameter_2_2, above=0.25cm of qwmult1](qw1) {};
\node [output2mat2, right=1.3cm of qwmult1](qyy1) {};
\draw [line width=0.1mm] ($(qw1.north east) + (0.1,0) $ ) -- ($(qw1.south east) + (0.1,0.0)$); % vertical line
\draw [line width=0.1mm] ($(qw1.north east) + (0.13,0) $ ) -- ($(qw1.north east) + (+0.07,0)$); % top tick
\draw [line width=0.1mm] ($(qw1.south east) + (0.13,0) $ ) -- ($(qw1.south east) + (+0.07,0)$); % bottom tick
\node [right=0.0cm of qw1]()[]{\tiny $^{6}$}; % right label
\node[left=-0.15cm of qw1] {\tiny $^{W^{(2)}_1}$};

% Edges
\draw ($(yy1.east) + (0.2em, 0em)$) edge[out=0,in=180,->] (qmult1);
\draw[-{>}] (qmult1) -- (qwmult1);
\draw[-{>}] (qw1) -- (qwmult1);
\draw (qwmult1) edge[out=0,in=180,->] (qyy1);


% POW 2
\node [draw, below right=1.1 and 0.5cm of yy1](qmult2) {$\times$};
\node [below=0cm of qmult2] (qa2) {$\widehat{A}^2$};
\node [draw, right=1cm of qmult2](qwmult2) {$\times$};
\node [parameter_2_3, above=0.25cm of qwmult2](qw2) {};
\draw [line width=0.1mm] ($(qw2.north east) + (0.1,0) $ ) -- ($(qw2.south east) + (0.1,0.0)$); % vertical line
\draw [line width=0.1mm] ($(qw2.north east) + (0.13,0) $ ) -- ($(qw2.north east) + (+0.07,0)$); % top tick
\draw [line width=0.1mm] ($(qw2.south east) + (0.13,0) $ ) -- ($(qw2.south east) + (+0.07,0)$); % bottom tick
\node [right=0.0cm of qw2]()[]{\tiny $^{3}$}; % right label
\node[left=-0.15cm of qw2] {\tiny $^{W^{(2)}_2}$};

% Edges
\draw ($(yy1.east) + (0.2em, 0em)$) edge[out=0,in=180,->] (qmult2);
\draw[-{>}] (qmult2) -- (qwmult2);
\draw[-{>}] (qw2) -- (qwmult2);



%% OUTPUTS

\node [output1mat2, above=0.1em of qyy1](qyy) {};
\draw (qwmult) edge[out=0,in=180,->] (qyy);
\node [output3mat2, below=0.1em of qyy1](qyy2) {};
\draw (qwmult2) edge[out=0,in=180,->] (qyy2);


\draw [line width=0.1mm] ($(qyy.north west) + (0,0.1) $ ) -- ($(qyy.north east) + (0,0.1)$); % horizontal line
\draw [line width=0.1mm] ($(qyy.north west) + (0,0.07) $ ) -- ($(qyy.north west) + (0,0.13)$); % left tick
\draw [line width=0.1mm] ($(qyy.north east) + (0,0.07) $ ) -- ($(qyy.north east) + (0,0.13)$); % bottom tick
\node [above=-0.05cm of qyy]()[]{\tiny $^n$}; % top label

\draw [line width=0.1mm] ($(qyy.north east) + (0.1,0) $ ) -- ($(qyy2.south east) + (0.1,0.0)$); % vertical line
\draw [line width=0.1mm] ($(qyy.north east) + (0.13,0) $ ) -- ($(qyy.north east) + (0.07,0)$); % top tick
\draw [line width=0.1mm] ($(qyy2.south east) + (0.13,0) $ ) -- ($(qyy2.south east) + (0.07,0)$); % bottom tick
\node [right=0cm of qyy1]()[]{\tiny $^{12}$}; % left label


\end{tikzpicture}



==> figs/misc/ourmodel.tex <==
%% Creator: Inkscape inkscape 0.92.2pre0, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'kipf.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{472.39506759bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,.9)%
    \newcommand*{\bigs}[1]{\scalebox{1.7}{\ensuremath#1}}

    \put(0,0.17){\includegraphics[width=1.05\unitlength,page=1]{figs/ourmodel1.pdf}}%
    
    {\fontsize{100pt}{120pt} \put(0.48,0.15){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$H^{(i+1)}$ }}}}%

    {\fontsize{100pt}{120pt} \put(-0.02,0.0){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$H^{(i+1)} = \sigma
    \bigs(\hat{A}^0 H^{(i)} W_0^{(i)} \bigs|\hat{A}^1  H^{(i)} W_1^{(i)}\bigs|\ldots\bigs)$  }}}}%
  \end{picture}%
\endgroup%


==> figs/misc/ourstikz.tex <==
\begin{tikzpicture}[scale=0.8, transform shape]
\definecolor{paramcolor}{HTML}{50ae55}
\definecolor{inputcolor}{HTML}{fd9727}
\definecolor{outputcolor}{HTML}{f1453d}

\tikzset{
	inputmat/.style = {rectangle, draw=inputcolor!70, fill=inputcolor!40, thick, minimum width=1.4cm, minimum height = 1cm},
	output1mat/.style = {rectangle, draw=black!0, fill=outputcolor!70, line width=0, inner sep=0pt, minimum width=0.2cm, minimum height = 1.0cm},
	output2mat/.style = {rectangle, draw=black!0, fill=outputcolor!30, line width=0, inner sep=0pt, minimum width=0.2cm, minimum height = 1.0cm},
	output3mat/.style = {rectangle, draw=black!0, fill=outputcolor!50, line width=0, inner sep=0pt, minimum width=0.2cm, minimum height = 1.0cm},
	thickermat/.style = {rectangle, draw=black!50, fill=black!20, thick, minimum width=1.4cm, minimum height = 1cm},
	thinmat/.style = {rectangle, draw=black!50, fill=black!20, thick, minimum width=0.2cm,
		minimum height = 1cm},
	parameter/.style = {rectangle, draw=paramcolor!70, fill=paramcolor!40, thick, minimum width=0.2cm, minimum height = 1.4cm},
}
\node [inputmat,anchor=south](x) [draw] {}; 
\node [right=-0.4em of x] (xlabel) {$H^{(i-1)}$};

%\node [below of=x](xlabel) {$H^{(l)}$}

\draw [decorate,decoration={brace,amplitude=5pt,mirror,raise=1ex}]
  ($(x.south west)+(-0.5em, 0.6em)$) -- ($ (x.south east)+(0.5em, 0.6em) $) node[midway,yshift=0em]{};



\node [draw, below left=0.5cm and 1.3cm of x](mult) {$\times$};
\node [left=0.15cm of mult] (a) {$\widehat{A}^0$};
%\node [thickermat, below of=mult](ax) [draw] {}; 
\node [draw, below of=mult](wmult) {$\times$};
\node [parameter, right =0.25cm of wmult](w1) {};
\node [below right=-0.6cm and -0.14cm of w1](wl) {$W^{(i)}_0$};
%\node [output1mat, below of=wmult](y1) {};

\node [draw, below=0.5cm of x](mult2) {$\times$};
\node [left=0.15cm of mult2] (a2) {$\widehat{A}^1$};
%\node [thickermat, below of=mult2](a2x) [draw] {}; 
\node [draw, below of=mult2](wmult2) {$\times$};
\node [parameter, right =0.25cm of wmult2](w2) {};
\node [below right=-0.6cm and -0.14cm of w2](wl) {$W^{(i)}_1$};
%\node [output2mat, below of=wmult2](y2) {};


\node [draw, below right=0.5cm and 1.3cm of x](mult3) {$\times$};
\node [left=0.15cm of mult3] (a3) {$\widehat{A}^2$};
%\node [thickermat, below of=mult3](a3x) [draw] {}; 
\node [draw, below of=mult3](wmult3) {$\times$};
\node [parameter, right =0.25cm of wmult3](w3) {};
\node [below=-0.1cm of w3](wl) {$W^{(i)}_2$};
%\node [output3mat, below of=wmult3](y3) {};


%\node [draw, below of=y2](concat) {concatenate};


\node [output2mat, below=1.3cm of wmult2](yy2) {};
\node [output1mat, left=0.1em of yy2](yy1) {};
\node [output3mat, right=0.1em of yy2](yy3) {};
\node [below=-0em of yy2] (xlabel) {$H^{(i)}$};

\draw [decorate,decoration={brace,amplitude=3pt,mirror,raise=1ex}]
  ($(yy1.south west)+(-0.5em, 0.6em)$) -- ($ (yy3.south east)+(0.5em, 0.6em) $) node[midway,yshift=0em]{};

\draw ($(x.south) + (0em, -0.3em)$) edge[out=270,in=90,->] (mult);
\draw[-{>}] (a) -- (mult);
\draw[-{>}] (mult) -- (wmult);
\draw[-{>}] (w1) -- (wmult);
\draw (wmult) edge[out=270,in=90,->] (yy1);

\draw ($(x.south) + (0em, -0.3em)$) edge[out=270,in=90,->] (mult2);
\draw[-{>}] (a2) -- (mult2);
%\draw[-{>}] (mult2) -- (a2x);
\draw[-{>}] (mult2) -- (wmult2);
\draw[-{>}] (w2) -- (wmult2);
\draw  (wmult2) edge[out=270,in=90,->] (yy2);


\draw ($(x.south) + (0em, -0.3em)$) edge[out=270,in=90,->] (mult3);
\draw[-{>}] (a3) -- (mult3);
%\draw[-{>}] (mult3) -- (a3x);
\draw[-{>}] (mult3) -- (wmult3);
\draw[-{>}] (w3) -- (wmult3);
\draw  (wmult3) edge[out=270,in=90,->] (yy3);
%\draw[-{>}] (y1) -- (yy1);
%\draw[-{>}] (y2) -- (yy2);
%\draw[-{>}] (y3) -- (yy3);
%\draw[-{>}] (concat) -- (yy2);
\end{tikzpicture}

